Functional Risk Minimization

The field of Machine Learning has changed significantly since the 1970s. However, its most basic principle, Empirical Risk Minimization (ERM), remains unchanged. We propose Functional Risk Minimization~(FRM), a general framework where losses compare functions rather than outputs. This results in better performance in supervised, unsupervised, and RL experiments. In the FRM paradigm, for each data point $(x_i,y_i)$ there is function $f_{\theta_i}$ that fits it: $y_i = f_{\theta_i}(x_i)$. This allows FRM to subsume ERM for many common loss functions and to capture more realistic noise processes. We also show that FRM provides an avenue towards understanding generalization in the modern over-parameterized regime, as its objective can be framed as finding the simplest model that fits the training data.

==> preamble_commands.tex <==
% KK 1
% Moved to main
% \usepackage{amsthm}
% \usepackage{bbm}
% \usepackage{ stmaryrd }


\input{variables.tex}

% KK 2
\newtheorem{assumption}{Assumption}
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{corollary}{Corollary}[theorem]
%\newtheorem{lemma}[theorem]{Lemma}
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\DeclareMathOperator{\BN}{BN}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\need}{{\normalfont{\text{tailor}}}}
\newcommand{\cont}{{\normalfont{\text{cont}}}}
\newcommand{\un}{{\normalfont{\text{un}}}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\thetax}{{\theta_x}}
\newcommand{\thetaxi}{{\theta_{x_i}}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\zetat}{\tilde \zeta}

\newcommand{\suploss}{\mathcal{L}^{\normalfont{\textrm{sup}}}}
\newcommand{\unsuploss}{\mathcal{L}^\textrm{unsup}}
\newcommand{\tailorloss}{\mathcal{L}^{\normalfont{\textrm{tailor}}}}

%\newcommand{\tailor}{\textrm{tailor}}
\newcommand{\tailor}{\tau}
\newcommand{\tailoredhypoth}{f_{\tailor(\hat{\theta}, x)}}


%\usepackage{amsmath}
%\DeclareMathOperator*{\argmax}{\arg\!\max}
%\DeclareMathOperator*{\argmin}{\arg\!\min}

\newcommand\ex[2]{#1^{(#2)}}
%\newcommand{\dtrain}{\mathcal{D}_{train}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bR}{\mathbb{R}}
%\usepackage{bbold}
\newcommand{\bOne}{1}
\newcommand\BOne[1]{1\llbracket #1 \rrbracket}
\newcommand\metric[2]{\mathcal{M}\left({#1},{#2}\right)}
\newcommand\loss[2]{\mathcal{L}\left({#1},{#2}\right)}
\newcommand{\Inp}{\mathcal{X}}
\newcommand{\Out}{\mathcal{Y}}
\newcommand{\supdata}{((x_i, y_i))_{i=1}^n}
\newcommand{\unsupdata}{(\ex{x}{j})_j}
\newcommand{\unsupdatum}{\ex{x}{j}}
\newcommand{\transoutput}{(\ex{\hat{y}}{j})_j}
\newcommand{\supalg}{\mathcal{A}}
\newcommand{\transalg}{\mathcal{T}}
 \newcommand{\lpk}[2][]{\todo[inline,linecolor=orange,backgroundcolor=orange!25,bordercolor=orange,#1]{lpk: #2}}
 \newcommand{\longname}{adaptive transduction }
 \newcommand{\shortname}{{\sc adatran}}
 \newcommand{\lonline}{\mathcal{L}_\text{unsup}}
 \newcommand{\loffline}{\mathcal{L}_\text{sup}}
%\newcommand\argmax[1]{{\rm arg}\max_{#1}}
%\newcommand\argmin[1]{{\rm arg}\min_{#1}}
\newcommand{\method}{{\sc CNGrad}}
\newcommand\expectation[2]{\mathbb{E}_{#1}\left[#2\right]}


\definecolor{darkolivegreen}{rgb}{0,.8,0.}%{0.03, 0.5, 0.08} %lo peta
%\newcommand{\greenx}[]{\textbf{\textcolor{darkolivegreen} x}} %: 
\newcommand{\greenx}{\textbf{\textcolor{darkolivegreen} x}} %TODO: Maria
\newcommand{\greenxi}{\textbf{$\textcolor{darkolivegreen} x_i$}}

